Influence of the distribution of the properties of permanent magnets on the field homogeneity of magnet assemblies for mobile NMR

We optimised the magnetic field homogeneity of two canonical designs for mobile microfluidic NMR applications: two parallel magnets with an air gap and a modified Halbach array. Along with the influence of the sample length, general design guidelines will be presented. For a fair comparison the sensitive length of the sample has been chosen to be the same as the gap size between the magnets to ensure enough space for the transmitting and receiving unit, as well as basic electric shimming components. Keeping the compactness of the final device in mind, a box with an edge length 5 times the gap size has been defined, in which the complete magnet configuration should fit. With the chosen boundary conditions, the simple parallel cuboid configuration reaches the best homogeneity without active shimming (0.5$\mathrm{B_{s}}$, 41 ppm), while the Pseudo-Halbach configuration has the highest field strength (0.9$\mathrm{B_{s}}$, 994 ppm), assuming perfect magnets. However, permanent magnet configurations suffer from imperfections, such as magnetisation, fabrication and positioning errors, which results in worse magnetic field homogeneities than expected from simulations using a fixed optimised parameter set. We present a sensitivity analysis for a magnetic cube and the results of studies of the variations in the magnetisation and angle of magnetisation of magnets purchased from different suppliers, composed of different materials and coatings, and of different sizes. We performed a detailed Monte Carlo simulation on the effect of the measured distribution of magnetic properties on the mentioned configurations. The cuboid design shows a mean homogeneity of 430 ppm (std dev. 350 ppm), the Pseudo-Halbach has a mean homogeneity of 1086 ppm (std dev. 8 ppm).

==> includes/TEX_headerAM.tex <==
% Tweak
\newcommand{\ruledtabular}{}%

% Double space
\usepackage{setspace}
\doublespacing

%General
\usepackage[pdftex]{hyperref}
\hypersetup{bookmarksnumbered=true}
\hypersetup{bookmarksopen=true}
\hypersetup{bookmarksopenlevel=2}
\usepackage{doi}
% Text
\hypersetup{colorlinks=true}
\hypersetup{linkcolor=black}
\hypersetup{citecolor=black}
\hypersetup{filecolor=black}
\hypersetup{menucolor=black}
\hypersetup{urlcolor=black}

% Define colors
\usepackage{color}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,0.5}
\definecolor{brown}{rgb}{0.98,0.92,0.73}
\definecolor{red}{rgb}{1,0,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{purple}{rgb}{1,0,1}
\definecolor{gray}{rgb}{0.8,0.8,0.8}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\definecolor{gold}{rgb}{1.,0.84,0.}

% Figures
\usepackage{graphicx}
%\usepackage{subcaption} % Incompatible with RevTex, Leon
\usepackage{caption}
\captionsetup{font=small,format=default,textfont=it}

% Units
\usepackage[]{siunitx}
\sisetup{range-units=single}
\sisetup{separate-uncertainty}
\sisetup{repeatunits=false}

% Math mode
\usepackage{mathptmx}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{nicefrac}

% Latexdiff
\newenvironment{DIFnomarkup}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Extra/changed functions %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\narrowfigurewidth{0.6\columnwidth}
\def\figurewidth{0.8\columnwidth}
\def\widefigurewidth{\columnwidth}

%comment-list
\newif\ifcmtr
\cmtrtrue
%\cmtrfalse
\ifcmtr %  Highlight comment (and hide it when necessary)
\newcommand{\cmtr}[1]{ %
   [\color{red} \textbf{#1} \normalcolor]%
}%
\else
\newcommand{\cmtr}[1]{ %
}% 
\fi

\ifcmtr %  Highlight comment (and hide it when necessary)
\newcommand{\cmtrla}[1]{ %
   [\color{blue} \textbf{#1} \normalcolor]%
}%
\else
\newcommand{\cmtrla}[1]{ %
}% 
\fi

\ifcmtr %  Highlight comment (and hide it when necessary)
\newcommand{\cmtrth}[1]{ %
   [\color{purple} \textbf{#1} \normalcolor]%
}%
\else
\newcommand{\cmtrth}[1]{ %
}% 
\fi

\ifcmtr %  Highlight comment (and hide it when necessary)
\newcommand{\cmtrpl}[1]{ %
   [\color{green} \textbf{#1} \normalcolor]%
}%
\else
\newcommand{\cmtrpl}[1]{ %
}% 
\fi
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Turbulator"
%%% End:


==> sections/Discussion.tex <==
\section{Discussion}

Discussion goes here


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Dumbbell"
%%% End:


==> sections/ResultsYannick.tex <==
\section{Results and Discussion}
\label {sec: Results}
\subsection{Magnet variation measurements}

We have measured the variations in the magnetization and magnetization angle 
of magnets obtained from different companies (Supermagnete, HKCM and
Schallenkammer Magnetsysteme), compositions (NdFeB N45, NdFeB N42,
Sm2Co17 YXG28, Sm2Co17 YXG26H), coatings (Ni-Cu-Ni, Ni-Cu, Ni, no
coating), and sizes (cylinders with a diameter of \SI{45}{} and
height of \SI{30}{mm} or cubes of \SI{7x7x7}{mm}). An overview is
given in Table~\ref{tab3} \footnote{The values between brackets are
	the absolute standard errors of the last shown digits.}.

\begin{figure} 
	\centering	\includegraphics[width=1\linewidth]{images/cdfmeanevery1000V3.pdf}
	\caption{Measured cumulative distribution of the field direction for a range of commercial magnets. The black line indicates our sensitivity limit. The sensitivity limit has been obtained from measuring \num{50} times the same magnet, indicated by the black line. We measured \num{10} different magnets with a diameter of $d$=\SI{45}{mm} and a height of $h$=\SI{30}{mm} (orange), and \num{50} magnets with a size of \SI{7x7x7}{mm} for each of the other kinds of material or manufacturer. On average, commercial magnets have a magnetization variation of less than \SI{1}{\percent}.}
	\label{fig10}
\end{figure}

\begin{figure} 
	\centering
	\includegraphics[width=1\linewidth]{images/distributionsangleerror4.pdf}
	\caption{Measured cumulative distribution of the field
		direction for a range of commercial magnets. On average,
		commercial magnets have a field direction variation of less
		than \ang{1}. The line indicated `Measurement error'
		shows a standard deviation of \ang{0.7}.}
	\label{fig11}
\end{figure}

% ruledtabular breaks the S option of siunitx:
% https://tex.stackexchange.com/questions/267868/does-ruledtabular-environment-from-revtex4-1-break-the-s-column-in-siunitx

\begin{table}
  \centering
  \caption{Measured variations in magnetization and magnetization angle
    of magnets with different materials, coatings, sizes and
    manufacturers.\label{tab3}}
  \begin{tabular*}{0.8\columnwidth}{l@{\extracolsep{\fill}}SS}
    \hline
    \hline
    Magnet &  {$\frac{B_\text{std}}{B_\text{mean}}[\si{\percent}]$}
    & { $ \phi $ [\si{\degree}] }\\
    \noalign{\vskip 0.5mm} % To avoid subscript touching line 
    \hline
    Su45Nd45NCN & 0.7(3) & 0.0(1)\\ 
    Su7Nd42NCN   & 0.8(2) & 0.7(2)\\ 
    Su7Nd42NC     & 0.6(3) & 0.0(1)\\ 
    HK7Nd35N       & 0.3(3) & 0.4(2)\\ 
    HK7Sm28N      & 1.0(3) & 0.2(1)\\ 
    Sc7Sm26          & 1.6(2) & 1.0(2)\\
    \hline
    \hline
  \end{tabular*}  
\end{table}

%\begin{table}[]
%	\centering
%	\caption{Measured magnetization and magnetization angle variations of magnets with different materials, coatings, sizes and manufacturers. The values between brackets are the absolute standard errors of the last shown digits.}
%	%	\resizebox{\columnwidth}{!}{%
%	\begin{tabular}{cccccc}
%		Magnet &  $\frac{B_{std}}{B_{mean}}[\%]$ & $ \phi $ [\degree] \\
%	    \hline
%		Su45Nd45NCN & 0.69(31) & 0.00(13) 	\\ 
%		Su7Nd42NCN  & 0.75(24) & 0.68(17) 	\\ 
%		Su7Nd42NC   & 0.63(25) & 0.00(12)	\\ 
%		HK7Nd35N    & 0.33(27) & 0.40(15) 	\\ 
%		HK7Sm28N    & 1.03(32) & 0.20(13)	\\ 
%		Sc7Sm26     & 1.55(17) & 1.07(20)
%	\end{tabular}
%	%	}
%	
%	
%	\label{tab3}
%\end{table}

On average, the magnetization varies by 1\% of $B_\text{mean}$
(Fig.~\ref{fig10}). The cylindrical magnet, which has a more than
\SI{50}{} times higher magnetic volume than the cubes, shows roughly the
same variation in magnetization. From this, we can conclude that
inaccuracies in the dimensions are not the main cause of the variation in
the magnetization. The uncoated Sm2Co17 shows a higher variation in
magnetization than the coated magnets, which could be caused by oxidation
or small damage to the magnet since unprotected sharp edges of
magnets tend to break off easily. Different coatings do not show a
clear trend regarding the magnetization standard variation or the
variation in the magnetisation angle. The offset angle varies on average by
less than \SI{1}{\degree} (Fig.~\ref{fig11}). There is no clear
relation between the variation in magnetization strength or
orientation and material, coating or manufacturer. 

\subsection{Comparison of designs}
\subsubsection{Optimization procedure}

To optimize the magnet configurations, the field inhomogeneity of its
\textit{z}-component was defined as the root mean square of the
difference between the mean field $B_\text{mean}$ and the field along the
sample $B_0$ with length $s$ related to the mean field:
\begin{align}
\dfrac{{\frac{1}{s}
		\int_{0}^{s}\sqrt{(B_0-B_\text{mean})^{2}}}dx}{B_\text{mean}}  \nonumber
\end{align}

\begin{figure}  
	\centering
	\includegraphics[width=1\linewidth]{images/CuboidW3776V3.pdf}
	\caption 
	{Field profile of the cuboid configuration as a function of the relative distance from the centre between the magnets. In the optimized situation for a sample size equal to the gap size, the field in the centre equals the field at the edge ($x$ = 0.5\textit{d}).}
	\label{fig2}
	\vspace{4ex}
\end{figure}
For a better understanding of the different magnet configurations, we start with a description of the cuboid case. The cuboid configuration can be found in Fig.~\ref{fig1}. Fig.~\ref{fig2} shows the magnetic field along the sample of the optimized cuboid configuration, in which the field is the same in the centre and at the edge of a sample. The field is symmetric, showing a valley in the middle and two peaks in the directions of the edges. After those maxima, the field decreases with the distance to the centre.


\begin{figure} 
	\centering
	\includegraphics[width=1\linewidth]{images/SamplesizeGapV3.pdf}
	\caption{Field inhomogeneity and field as a function of the sample size for the cuboid configuration. The homogeneity has been optimized for a sample size equal to the gap. With increasing sample size, both the field and the field inhomogeneity increase theoretically (region I). The field reaches a local maximum of \num{0.50041}$B_\text{s}$ at a distance of \num{0.71}$d$ from the centre. Above this distance the homogeneity of the sample stays approximately the same (region II). When the sample size increases more than the gap size, the inhomogeneity strongly increases (region III). Hence, to optimize the homogeneity of the cuboid magnet configuration, the field difference between the centre and the sample edge needs to be minimized.} 
	\label{fig3}
	\vspace{4ex}
\end{figure}

Fig.~\ref{fig3} shows how the field homogeneity develops with increasing sample size while keeping the previously optimized parameter set constant. Three regions can be seen. In the first one the field increases from \num{0.50035}$B_\text{s}$ to \num{0.50041}$B_\text{s}$, which means that the minimum field of \num{0.50035}$B_\text{s}$ stays the same while the maximum field is increasing until it reaches its global maximum, hence the inhomogeneity is also increasing. In the second region the inhomogeneity stays almost constant. In the third region the field decreases below the previous minimum, which results in a drastic increase of the inhomogeneity. Because of this, the lowest inhomogeneity between two points can be either reached keeping the sample as short as possible or when the field difference at the sample edges and the middle are the same. This information is important for the following optimization processes. 


\paragraph{Cuboid}

The cuboid configuration (Fig.~\ref{fig1}) consists of two parallel cuboid magnets. The length $L$ of the whole configuration has been chosen to be five times the gap size $d$. The width $W$ was used to tune the field in between the magnets. This subsection will show how to optimize a cuboid configuration using its width to tune the homogeneity of the field. From the previous section we know that we have to find a width for which the field in the centre and at the sample edge is the same.

\begin{figure} 
	\centering
	\includegraphics[width=1\linewidth]{images/CuboidhomogeneitystrengthV4.pdf}
	\caption
	{Field strength in the middle of the configuration and
		difference of the field centre and the edge of the sample,
		both as functions of the ratio of the cuboid width over the length. The
		field increases up to \num{0.54}$B_\text{s}$ at a cuboid width
		of \num{3.0375} times the gap size. The inset shows the
		field difference dropping to zero at a width/gap ratio of
		\num{4.72}.}
	\label{fig4}
\end{figure}

Fig.~\ref{fig4} shows that the magnetic field in the centre increases 
to its maximum of \num{0.54}$B_\text{s}$ at a width of
\num{3.0375}$d$. Increasing the width further results in a reduction
of the magnetic field, caused by the larger distance from the 
edges of the magnet to the centre. The difference between the magnetic field in the
centre and that at the sample edge increases until it reaches a maximum, when the
width equals the gap size. From this point the difference decreases
until it reaches a minimum at a width/gap ratio of \num{4.72}. The stray field at a
distance equal to the gap size is \num{0.24}$B_\text{s}$.

\paragraph{Pseudo-Halbach}
The pseudo-Halbach configuration consists of
eight magnets, arranged in such a way that the field in the bore is
enhanced while the external stray field is minimized. The magnets have
a fixed dimension $d \times d \times 5d$. To tune the homogeneity,
the position of the magnets in the corners is fixed, while the other
magnets are spread out over a distance $C$  (Fig.~\ref{fig1}). The
width starts at $W = 3d$ to ensure a minimum bore width $d$ and ends
at $W= L$, due to the previously chosen boundary conditions.  

\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{images/Halbach3.pdf}
	\caption{Spreading the middle magnets has been used to change
		the normalized field strength and field difference. At a
		spread parameter $C = 0$, a minimal field difference of
		\SI{3365}{ppm} and a field strength of \num{0.90}$B_\text{s}$
		can be reached.}
	\label{fig5}
	\vspace{4ex}
\end{figure}

Spreading the configuration increases the distance of the middle magnets,
which produces a decreased magnetic field strength
(Fig.~\ref{fig5}). With this configuration the convex field profile
has no chance to change to a concave profile. Therefore a minimum can
not be reached. With the most compact magnet arrangement, a field of
\num{0.9}$B_\text{s}$ and a field difference of \SI{3365}{ppm} can be
achieved. The stray field at a distance equal to the
gap size from the surface is \num{0.07}$B_\text{s}$.

%\FloatBarrier


\subsubsection{Influence of variations in the magnets}

\paragraph{Choice of parameters to vary}

We calculated the influence on the magnetic field of a variation of
the dimensions, position, and tilt of the magnets, as well as in the magnetization
strength and angle (shown in Fig.~\ref{fig8}). We consider the field
components $B_{x}, B_{y}, B_{z}$ at a point above the centre of the
top (north) face, at a height of 10\% of the length $a$ of the edge of the magnet.

Besides calculations, we also measured the magnetization and
magnetization angle of magnets with different sizes, materials,
coatings, and manufacturers. These measured variations are used for 
Monte Carlo simulations to estimate the field homogeneity of a
cuboid magnet and a pseudo-Halbach magnet configuration after
assembly.

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{images/Cuboidangle.pdf}
	\caption{Schematic drawing of a cubic magnet. The arrows
		indicate the direction of magnetization. $\phi$ shows the
		total offset angle, $\theta$ the offset direction in
		cylindrical coordinates.}
	\label{fig7}
\end{figure}

\begin{figure} 
	\centering
	\includegraphics[width=1\linewidth]{images/BdistanceV3.pdf}
	\caption{Magnetic field ($x,y,z$) above a cuboid magnet with
		the edge length $a$ along the $x$-axis at a distance of
		\num{0.1}$a$.}
	\label{fig8}
\end{figure}

As can be seen in Fig.~\ref{fig8}, the cubic magnet, magnetized in
the $z$-direction, shows no field in the $y$-direction ($B_{y}$) along the
$x$-axis at a distance of \num{0.1}$a$ from the surface. The field
$B_{x}$ is zero in the centre of the magnet and rises linearly with a
slope of \num{0.04}$B_\text{s}/a$ in the positive
$x$-direction, with $B_\text{s}$ the saturation magnetization of the
magnet material [T]. The field $B_{z}$ is \num{0.357}$B_\text{s}$ in the centre which drops to \num{0.355}$B_\text{s}$ at $x=0.1a$. 


Table~\ref{tab2reduced} shows the sensitivity matrix of the magnetic field in
the $x$ and $z$-directions on the $x$-axis at a distance of 0.1$a$,
given as percentages of $B_\text{s}$. Table~\ref{tab2} in appendix shows a more extended matrix, including $B_{y}$ and the field at $x$=0.1$a$. Parameters related to the sizes 
have been varied by \SI{10}{\percent} of the length of the edge of the cube. Parameters related to the angle
have been varied by \SI{1}{\degree}. The
sensitivity matrix of the field in the $x$-direction shows that the field
strength changes proportionally with the magnetization. The magnet tilt
angle and the magnetization offset angle around the $x$-axis, as well as moving
the magnet in the $y$-direction, does not have any influence on the
magnetic field. A tilt or a magnetization offset angle around the
$y$-axis has a much more significant influence on the field: tilting
changes the field from \SI{0.61}{\percent} in the centre to \SI{0.51}{\percent} at $x=
0.1a$; the magnetic offset angle changes the field from \SI{-0.87}{\percent} in
the centre to \SI{-0.88}{\percent} at $0.1a$. Moving the magnet in
the $x$-direction has the biggest influence on $B_{x}$: \SI{-1.09}{\percent}
in the centre to \SI{-1.15}{\percent} at $0.1d$. Misplacements in other
directions and variations in the dimensions have a minor influence on the
field. The field in the $y$-direction is influenced by tilting the
magnet and a magnetization offset angle around the $x$-axis and moving
the magnet in the $y$-direction. The other parameters do not affect the
field. The field in the $z$-direction has a high dependency on the
distance to the magnet, twice as big as the change due to variations in the
magnetization. Tilting the magnet changes the field linearly
from \num{0} at $x$=$0$ to \SI{-0.48}{\percent} at $x$=$0.1a$. Other variables have
a rather small influence on the field.

Summarizing, the variations in the tilt and magnetization angle have a
significant influence when the rotational axis is perpendicular to
the observed axis. Variations in the placement of the magnet have a significant
influence if this variation is in the same direction as the observed
field. Variations in the dimensions have a relatively small influence on the
field at the observed locations compared to the other varied
parameters.

\newcommand{\standout}[1]{\color{blue} #1}
%\newcommand{\standout}[1]{\num{\textbf{#1}}} % DOES NOT WORK



\begin{table}
		\centering
	\caption{Sensitivity matrix of the magnetic field
		($B_x$,$B_z$), given in the change of
		$B_\text{s}$ at the same position in [\SI{}{\percent}] above the center of a cuboid magnet
		with the edge length $a$ at a distance of
		$0.1a$. Variations in the magnetization angle
		and tilting the magnet perpendicular to the simulated
		axis affect the magnetic field significantly. Placement errors have
		an influence if parallel to the field. }
	\begin{tabular}{ll@{\extracolsep{\fill}}SS}
		\hline 
		\hline
		& Variation & { $B_x$}  &{$B_z$}  \\
		\hline
		$M$ & 1\% & 0.00  & \standout{1.00}  \\
		\noalign{\vskip 0.7mm} % set off to group rows
		tilt $x$ & \SI{1}{\degree} & 0.00 & 0.00  \\
		tilt $y$ & \SI{1}{\degree} & \standout{0.61} &  0.00  \\
		\noalign{\vskip 0.7mm} % set off to group rows
		$\phi$ ($\theta$=~\SI{0}{\degree}) & \SI{1}{\degree} & 0.00  & 0.00 \\
		$\phi$ ($\theta$=\SI{90}{\degree}) & \SI{1}{\degree} & \standout{-0.87} & 0.00  \\
		\noalign{\vskip 0.7mm} % set off to group rows
		$x$ & 0.1$a$ & \standout{-1.09} & 0.00 \\
		$z$ & 0.1$a$ & 0.00 & \standout{-2.17}\\
		\hline \hline
	\end{tabular}
	\label{tab2reduced}
\end{table}


\begin{table*}
%	\centering
	\caption{Sensitivity matrix of the magnetic field
		($x$,$y$,$z$), given in the change of
		$B_\text{s}$ at the same position in [\SI{}{\percent}] above a cuboid magnet
		with the edge length $a$ along the $x$-axis at a distance of
		$0.1a$. Variations in the magnetization angle
		and tilting the magnet perpendicular to the simulated
		axis affect the magnetic field significantly. Placement errors have
		an influence if parallel to the field. Variations in the dimensions have a
		minor effect.}
	\begin{tabularx}{1\textwidth}{ll@{\extracolsep{\fill}}SSSSSS}
		\hline 
		\hline
		& & \multicolumn{2}{c}{$B_{x}$} & \multicolumn{2}{c}{$B_{y}$} &
		\multicolumn{2}{c}{$B_{z}$} \\
		\cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} 
		& Variation & {$x=0$} & {$x=0.1a$} &{$x=0$} & {$x=0.1a$} &{$x=0$} & {$x=0.1a$} \\
		\hline
		$M$ & 1\% & 0.00 & \standout{1.10} & 0.00 & 0.00 & \standout{1.00} & \standout{0.99} \\
		\noalign{\vskip 0.7mm} % set off to group rows
		tilt $x$ & \SI{1}{\degree} & 0.00 & 0.00 & \standout{-0.61} & \standout{-0.62} & 0.00 & 0.00 \\
		tilt $y$ & \SI{1}{\degree} & \standout{0.61} & \standout{0.51} & 0.00 & 0.00 & 0.00 & \standout{-0.48} \\
		\noalign{\vskip 0.7mm} % set off to group rows
		$\phi$ ($\theta$=~\SI{0}{\degree}) & \SI{1}{\degree} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
		$\phi$ ($\theta$=\SI{90}{\degree}) & \SI{1}{\degree} & \standout{-0.87} & \standout{-0.88} & \standout{-0.87} & \standout{-0.86} & 0.00 & 0.19 \\
		\noalign{\vskip 0.7mm} % set off to group rows
		$x$ & 0.1$a$ & \standout{-1.09} & \standout{-1.15} & 0.00 & 0.00 & 0.00 & 0.10 \\
		$y$ & 0.1$a$ & 0.00 & 0.00 & \standout{1.09} & \standout{1.07} & 0.00 & 0.00\\
		$z$ & 0.1$a$ & 0.00 & -0.10 & 0.00 & 0.00 & \standout{-2.17} &\standout{-2.22} \\
		\noalign{\vskip 0.7mm} % set off to group rows
		height & 0.1$a$ & 0.00 & 0.02 & 0.00 & 0.00 & \standout{0.23} & \standout{0.23} \\
		depth & 0.1$a$ & 0.00 & \standout{-0.18} & 0.00 & 0.00 & -0.01 & 0.01 \\
		width & 0.1$a$ & 0.00 & 0.05 & 0.00 & 0.00 & -0.01 & -0.01 \\
		\hline \hline
	\end{tabularx}
	\label{tab2}
\end{table*}

%\begin{table}[]
%	\centering
%	\caption{Sensitivity matrix of the magnetic field ($x$,$y$,\textit{z}), given in the change of $\mathrm{B_\text{s}}$ at the same position in [\%] above a cuboid magnet with the edge length d along x-axis at a distance of 0.1\textit{d}. From this matrix we conclude that magnetization variations change the field proportionally. Magnetization-angle variations and tilting the magnet perpendicular to the simulated axis affect the magnetic field significantly. Placing errors have an influence, in case the direction is the same as the simulated field. Dimension variations have a minor influence on the magnetic field.
%	}
%	\resizebox{\columnwidth}{!}{%
%		\begin{tabular}{cccccccc}
%			&Variation & $B_{x}$($x$=0) & $B_{x}$($x$=0.1\textit{d}) & $B_{y}$($x$=0) & $B_{y}$($x$=0.1\textit{d}) & $B_{z}$($x$=0) & $B_{z}$(x=0.1d) \\ \hline
%			M & 1\% & 0.00 & 1.10 & 0.00 & 0.00 & 1.00 & 0.99 \\ 
%			tilt $x$ & 1\degree & 0.00 & 0.00 & -0.61 & -0.62 & 0.00 & 0.00 \\ 
%			tilt $y$ & 1\degree & 0.61 & 0.51 & 0.00 & 0.00 & 0.00 & -0.48 \\ 
%			$\phi$ ($\theta$ = 0 \degree) & 1\degree & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
%			$\phi$ ($\theta$ = 90 \degree)  & 1\degree & -0.87 & -0.88 & -0.87 & -0.86 & 0.00 & 0.19 \\ 
%			$x$ & 0.1\textit{d} & -1.09 & -1.15 & 0.00 & 0.00 & 0.00 & 0.10 \\ 
%			$y$ & 0.1\textit{d} & 0.00 & 0.00 & 1.09 & 1.07 & 0.00 & 0.00 \\ 
%			\textit{z} & 0.1\textit{d} & 0.00 & -0.10 & 0.00 & 0.00 & -2.17 & -2.22 \\ 
%			height & 0.1\textit{d} & 0.00 & 0.02 & 0.00 & 0.00 & 0.23 & 0.23 \\ 
%			depth & 0.1\textit{d} & 0.00 & -0.18 & 0.00 & 0.00 & -0.01 & 0.01 \\ 
%			width & 0.1\textit{d} & 0.00 & 0.05 & 0.00 & 0.00 & -0.01 & -0.01
%		\end{tabular}
%	}
%	
%	\label{tab2}
%\end{table}



\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{images/FieldZXZdiffdeg1deg0V4.pdf}
	\caption{Logarithmic plot of the field difference normalized to one-half
		of the sum of $B_z$ with an offset angle of \SI{0}{\degree} and \SI{1}{\degree}
		generated by a cubic magnet with an edge length of $a$. The field
		difference has its minimum right above, and right next to the
		magnet, along the $x$- and $z$-axes. A maximum can be found along a
		straight line with a slope of 0.7 $z$/$x$.}
	\label{fig9}
\end{figure}

Figure~\ref{fig9} shows a logarithmic plot of the field difference
normalized to one-half of the sum of $B_z$ with an offset angle of
\SI{0}{\degree} and \SI{1}{\degree} on the $xz$-plane. Right above ($z$-axis)
and next to the magnet ($x$-axis), the field is least affected by the
magnetization offset angle. 
The difference has its maximum along a line with slope \num{0.7}$z$/$x$.

\paragraph{Simulation of effect of variations in the magnet }

A Monte Carlo simulation ($n$=\num{50000}) of the homogeneity has been
performed with two input parameters for each magnet, both for the
cuboid and the pseudo-Halbach configuration. A normal distribution was
assumed, using our measurements of the standard deviations of
\SI{1}{\degree} in the magnetization angle and \SI{1}{\percent} of the
magnetization. No placement errors or dimensional errors were considered.

\begin{figure} 
	\centering
	\includegraphics[width=1\linewidth]
	{images/DistributionCuboidHalbachV3.pdf}
	\includegraphics[width=1\linewidth]
	{images/CDFHomogeneityeverynthV2.pdf}
	\caption{Density plot (top) and cumulative distribution
		function (bottom) of the Monte Carlo simulation for the cubic and
		Pseudo-Halbach configurations. The simulation shows that the
		Pseudo-Halbach configuration has a mean homogeneity of \SI{1086}{ppm}
		(standard deviation \SI{8}{ppm}), while the cuboid configuration
		reaches \SI{430}{ppm} (standard deviation \SI{350}{ppm}).}
	\label{fig12}
\end{figure}

Fig.~\ref{fig12} shows a distribution and probability plot of the
obtained homogeneities of the magnetic field in the $z$-direction
simulated by a Monte Carlo simulation. The mean homogeneity of the
cuboid configuration is \SI{430}{ppm}, the pseudo-Halbach configuration
achieves \SI{1086}{ppm}. However, the cuboid configuration has a high
spread in the homogeneity (standard deviation \SI{350}{ppm}) while
the pseudo-Halbach has a standard deviation of only \SI{8}{ppm}. With
a probability of \SI{94.4}{\percent}, both the cuboid configuration and
the pseudo-Halbach configuration obtain a homogeneity of \SI{1098}{ppm}
or better.  With a probability of \SI{10}{\percent}, the cuboid
configuration achieves \SI{64}{ppm} whereas the pseudo-Halbach achieves
not less than \SI{1076}{ppm}.

\begin{table}
	\centering
	\caption{Sensitivity matrix of the $z$-field at $x$=$0$ and
		$x$= $d/2$ for the pseudo-Halbach configuration}
	\begin{tabular}{lSSl}
		\hline
		\hline
		%\toprule
		%\toprule
		& {$B_z$ ($x=0$)} & {$B_z$ ($x=d/2$)} & \\ 
		\hline
		$M$ (total) & 902.237 & 899.209 & mT \\ 
		$M$ (top/bottom) & 1737 & 1743  &ppm \\ 
		$M$ (side) & 1515  & 1520 &ppm\\ 
		$M$ (corner) & 876  & 877 & ppm\\ 
		Angle (top/bottom) & 0 & 59 &ppm \\ 
		Angle (side) & 0 & 0 & ppm\\ 
		Angle (corner) & 0 & 81 & ppm \\
		\hline
		\hline
		%\bottomrule
		%\bottomrule
	\end{tabular}%
	\label{tab4}
\end{table}

\begin{table}
	\centering
	\caption{Sensitivity matrix of the
		$z$-field at $x$=0 and $x$= \textit{d}/2 for the
		cuboid-configuration }
	\begin{tabular}{lSSl}
		\hline
		\hline
		%\toprule
		%\toprule
		& {$B_z$ ($x=0$)} & {$B_z$ ($x=d/2$)} & \\ 
		\hline
		$M$ (total) & 499.301 & 499.301 & mT \\ 
		$M$ & 4998 & 4998 & ppm \\ 
		Angle & 0 & 985 & ppm \\
		\hline
		\hline
		%\bottomrule
		%\bottomrule
	\end{tabular}%
	\label{tab5}
\end{table}

\begin{table}
	\centering
	\caption{Magnetization angle related sensitivity matrix of the $z$-field at $x$=$0$ and
		$x$= $d/2$ for the pseudo-Halbach and cuboid configuration}
	\begin{tabular}{lSSl}
		\hline
		\hline
		%\toprule
		%\toprule
		& {$B_z$ ($x=0$)} & {$B_z$ ($x=d/2$)} & \\ 
		\hline
		Angle (top/bottom - Halbach) & 0 & 59 &ppm \\ 
		Angle (side - Halbach) & 0 & 0 & ppm\\ 
		Angle (corner - Halbach) & 0 & 81 & ppm \\
	    Angle (Cuboid)& 0 & 985 & ppm \\
		\hline
		\hline
		%\bottomrule
		%\bottomrule
	\end{tabular}%
	\label{tab45}
\end{table}


An indication of why the cuboid configuration has a much higher standard
deviation than the pseudo-Halbach configuration can be seen
from the sensitivity matrices of the $z$-field. We chose to show how
the field in the centre and at $x$=$d/2$ changes for a magnetization
difference of \SI{1}{\percent} and an offset magnetization direction
of \SI{1}{\degree} each in the direction which creates the highest
field difference at both locations. The Halbach configuration consists
of 8 magnets: 4 corner magnets, 2 at the side, and 1 each on top and
bottom. Adding up the sensitivity values of all the magnets results in a
difference of \SI{314}{ppm} between the $z$-field at $x$=0 and
$x$=$d/2$. The cuboid shows a significantly higher difference of
\SI{1970}{ppm}.

Regarding a single cubic magnet, the field difference, normalized to
one-half the sum of $B_z$, has a minimum right above and next to the
magnet. The difference increases with an increased distance from the
axis. Since the cuboid configuration has fewer
of magnets, the chance that all magnets have the same
deviation in their magnetization angle in the same direction is much higher than
for the pseudo-Halbach configuration.


\paragraph{Measurements of the effect of variations in the magnet on the homogeneity, for the cuboid and the pseudo-Halbach configurations}

\begin{table}
	\centering
	\caption{Measured homogeneity of cuboid and pseudo-Halbach configurations}
	\begin{tabular}{lS}
		\hline
		\hline
		%\toprule
		%\toprule
		& {Inhomogeneity}\\
		& $[$ppm$]$ \\
		\noalign{\vskip 0.5mm} % To avoid subscript touching line 
		\hline
		Cuboid 1 & 748(3) \\ 
		Cuboid 2 & 2250(3) \\ 
		Cuboid 3 & 1021(3) \\ 
		Pseudo-Halbach 1 & 1088(3) \\ 
		Pseudo-Halbach 2 & 1081(3) \\ 
		Pseudo-Halbach 3 & 929(3) \\
		\hline
		\hline
		%\bottomrule
		%\bottomrule
	\end{tabular}
	
	\label{tab6}
\end{table}


\begin{table}
	\centering
	\caption{Mean (standard deviation) of the homogeneity of the field
		in the $z$-direction of measured and simulated magnet
		configurations}
	\begin{tabular}{lSS}
		%\toprule
		%\toprule
		\hline
		\hline
		& {Measured } & {Simulated }\\
		& {Inhomogeneity} & {Inhomogeneity}\\
		&  {$[$ppm$]$} & {$[$ppm$]$} \\
		\noalign{\vskip 0.5mm} % To avoid subscript touching line
		\hline
		Cuboid & 1340(800) & 430(350) \\ 
		Pseudo-Halbach & 1032(90) & 1086(6) \\
		\hline
		\hline
		%\bottomrule
		%\bottomrule
	\end{tabular}
	\label{tab7}
\end{table}

Both configurations were assembled and measured three times. The
measurement results are shown in Table~\ref{tab6}. One can see a small
spread in the homogeneity of the pseudo-Halbach (mean value of
\SI{1032}{ppm} and standard deviation of \SI{90}{ppm}). A larger
spread was found for the cuboid configuration
(SI{1340}{} and \SI{800}{ppm}), see Table~\ref{tab7}.

Using the results of the Monte Carlo simulation from Fig.~\ref{fig12}, we can
calculate the likelihood of measuring a homogeneity of, for instance,
approximately \SI{1000}{ppm} or worse. For the cuboid configuration,
this is a relatively low likelihood of \SI{6.5}{\percent}, and even lower
(\SI{0.006}{\percent}) for the pseudo-Halbach configuration. However,
we measured inhomogeneities above \SI{1000}{ppm} on only three
realizations. It seems very likely that the inhomogenities are not only
caused by the spread in the properties of the magnets themselves, but also by
inaccuracies in the manufacturing of the entire assembly.

In general, the pseudo-Halbach configuration has a more predictable
field profile, which makes this design more favourable for industrial
applications than the cuboid configuration. Since shimming is needed
anyway, a measurement of the field profile is not necessary. We
therefore recommend restricting the use of the cuboid configurations
to research systems, where selecting the magnets and measuring the
final assembly is feasible.

\subsection{Comparison}

\subsubsection{General comparison}

\begin{table}
	\centering
	\caption{Comparison of magnetic properties of different magnet configurations.}
	\begin{tabular}{lSSS}
		\hline
		\hline
		%\toprule
		%\toprule
		& {$B_\text{max}$}  & {$B_\text{stray}$} & {$\Delta B_\text{rms}/B_\text{mean}$} \\
		& {$[B_\text{s}]$} & {$[B_\text{s}]$} & {$[$ppm$]$} \\
		\noalign{\vskip 0.5mm} % To avoid subscript touching line
		\hline
		Cuboid & 0.5 & 0.24 & 41  \\
		Pseudo-Halbach & 0.9 & 0.07 & 994 \\
		\hline
		\hline	
		%\bottomrule
		%\bottomrule
	\end{tabular}		
	\label{tab1}
\end{table}

Table~\ref{tab1} compares the major specifications of the two
configurations. The pseudo-Halbach configuration achieves
\num{0.9}$B_\text{s}$, a \num{1.8} times higher field than the Cuboid
configuration, while the stray field at a distance of $d$ from the
magnet surface is \num{0.07}$B_\text{s}$, which is \num{3.4} times lower.
In terms of homogeneity, the Cuboid configuration achieves a homogeneity
of \SI{41}{ppm}, which, compared to the pseudo-Halbach configuration,
is \num{24.2} times better.

\subsubsection{Influence of the sample length}

We optimized the homogeneity of the configuration for different sample
sizes, while keeping the outer boundary conditions the same.
Fig.~\ref{fig6} shows how the homogeneity changes with a smaller
ratio of the gap size to the sample size.


\begin{figure} 	
	\centering
	\includegraphics[width=1\linewidth]
	{images/ComparisonallhalbachcuboidrmsfitV3.pdf}
	\caption{Inhomogeneity of the magnetic field as a function of the
		sample length/gap ratio with a constant configuration width/gap
		ratio of \num{5}. For every sample size, the width of the cuboid
		configurations has been optimized to reach the lowest possible
		inhomogeneity. For a homogeneity reasonable for NMR applications
		of \SI{0.1}{ppm}, the sample length for a cuboid configuration
		needs to be $0.22d$, whereas it has to become unrealistically
		short ($0.01d$) for the pseudo-Halbach configuration.}
	\label{fig6}
\end{figure}

In every case, reducing the sample size yields a better homogeneity. The cuboid configuration can reach in theory \SI{0.01}{ppm} with a sample size of $0.22d$, while the pseudo-Halbach configuration needs an absurd sample length of $0.01d$ to reach this value. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Sensitivity"
%%% End:


==> sections/Theory.tex <==
\section{Theory}
Variables like this $z$, $h_\text{top}$.

\begin{equation}
  \label{eq:emc2}
  E=mc^2
\end{equation}

\noindent where $m$ is the mass of the object (\si{kg}), $c$ the speed
of light (\SI{3e8}{m/s}).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Dumbbell"
%%% End:

